Language model compression with weighted low-rank factorization

Factorizing a large matrix into small matrices is a popular strategy for model compression. Singular value decomposition (SVD) plays a vital role in this compression strategy, approximating a learned matrix with fewer parameters. However, SVD minimizes the squared error toward reconstructing the original matrix without gauging the importance of the parameters, potentially giving a larger reconstruction error for those who affect the task accuracy more. In other words, the optimization objective of SVD is not aligned with the trained model's task accuracy. We analyze this previously unexplored problem, make observations, and address it by introducing Fisher information to weigh the importance of parameters affecting the model prediction. This idea leads to our method: Fisher-Weighted SVD (FWSVD). Although the factorized matrices from our approach do not result in smaller reconstruction errors, we find that our resulting task accuracy is much closer to the original model's performance. We perform analysis with the transformer-based language models, showing our weighted SVD largely alleviates the mismatched optimization objectives and can maintain model performance with a higher compression rate. Our method can directly compress a task-specific model while achieving better performance than other compact model strategies requiring expensive model pre-training. Moreover, the evaluation of compressing an already compact model shows our method can further reduce 9% to 30% parameters with an insignificant impact on task accuracy.

==> additional/add.tex <==
\begin{align}
{g_i} = ({\sigma _{im - m + 1,...,}}{\sigma _{im}}) 
\label{equ:gi}\\
{{\bar \Sigma }_i} = [{g_1},...,{g_i} = \vec 0,...,{g_{r/m}}] \label{equ:sigmai}
\end{align}


The factorization of a rank-$r$ matrix $W$ retain only the $r$ columns of $U$ and $V$, associated with non-zero singular values: ${\sigma _1} \ge {\sigma _2} \ge  \cdots {\sigma _r} > 0$. 
The low-rank approximation with target rank $l$ is achieved by setting zeros to the  last $r-l$ singular values.
The reconstruction of matrix $A$ can also be viewed rank revealing decomposition:
\begin{equation}
    %A=\sum_{k=1}^r \sigma_k u_k v_k^T,
    ||W||_F=\sum_{k=1}^r \sigma_k^2
    \label{equ:rank_decomposition}
\end{equation}
where $u_k$ and $v_k$ is the $k$th column of $V$.\yh{I do not quite understand the notations here}
For $i<j$, column $i$ will be more important in the matrix reconstruction process than column $j$, since ${\sigma_i > {\sigma_j}}$. 
Ideally, setting $\sigma_i$ to zero is supposed to cause larger reconstruction error and result in worse final performance than setting $\sigma_j$ to zero. 
Therefore, 

==> iclr2022_app_backup.tex <==
\appendix
\section{Appendix}
You may include other additional sections here.

$U^*={{\hat I}^{ - 1}}\hat U\hat S$, and $V^*=\hat V$

Specifically, our evaluation datasets 2 single-tasks CoLA \needcite SST-2, 3 sentence similarity tasks MRPC QQP,
3 natural language inference taks: MNLI RTE QNLI.

%${{\bar S}_i} = diag(\begin{array}{*{20}{c}}{{\Sigma _1},}&{ \ldots ,}&{{\Sigma _{i - 1}},}&{0,}&{{\Sigma _{i - 1}},}&{ \ldots ,}&{{\Sigma _{r/g}}}\end{array})$

${{\bar S}_i} = diag \left({{\Sigma _1},}&{ \ldots ,}&{{\Sigma _{i - 1}},}&{0,}&{{\Sigma _{i - 1}},}&{ \ldots ,}&{{\Sigma _{r/g}}} \right)$

$\Sigma_i=diag(\sigma_i,...,\sigma_{i+g-1})$

we split singular values of matrix $W$ into $m$ groups, and each group contains $r/m$ elements. remove one group each time, and evaluate the performance drop and reconstruction error of the matrix recomposed by the $g-1$ groups. ${{\bar S}_i} = diag \left({{\Sigma _1},}&{ \ldots ,}&{{\Sigma _{i - 1}},}&{0,}&{{\Sigma _{i - 1}},}&{ \ldots ,}&{{\Sigma _{r/g}}} \right)$





==> iclr2022_relatedWork.tex <==
\section{Related Work}
equivalent optimization: \cite{chen2018groupreduce}\\

If we can get 250(or lower) rank without loss any acc.\\
SVD baseline for NLP:\cite{noach2020compressing}\\
Tinybert\\
Distillbert\\
BERT-PKD\\
BERT-of-Theseus \cite{xu-etal-2020-bert}\\


If we can get 125(or lower) rank without loss any acc.\\
Ladabert (SVD + irregular pruning): \cite{mao2020ladabert}

==> tabs_figs/app_fig1.tex <==
\begin{figure} [htbp]
  \begin{subfigure}[b]{.49\textwidth}
   \centering
   \includegraphics[width=\textwidth]{figures/app_mrpc_per.pdf}
       \caption{MRPC performance drop}
       \label{app:mrpc_per}
       \end{subfigure}
\begin{subfigure}[b]{.49\textwidth}
\includegraphics[width=\textwidth]{figures/app_mrpc_err.pdf}
\centering
  \caption{MRPC error}
   \label{app:mrpc_err}
\end{subfigure}
  \begin{subfigure}[b]{.49\textwidth}
   \centering
   \includegraphics[width=\textwidth]{figures/app_ner_perpdf.pdf}
       \caption{CoNLL-03 performance Drop}
       \label{app:ner_per}
       \end{subfigure}
\begin{subfigure}[b]{.49\textwidth}
\includegraphics[width=\textwidth]{figures/app_ner_err.pdf}
\centering
  \caption{CoNLL-03 Error}
   \label{app:ner_err}
\end{subfigure}
  \begin{subfigure}[b]{.49\textwidth}
   \centering
   \includegraphics[width=\textwidth]{figures/app_cola_per.pdf}
       \caption{COLA performance drop}
       \label{app:cola_per}
       \end{subfigure}
\begin{subfigure}[b]{.49\textwidth}
\includegraphics[width=\textwidth]{figures/app_cola_err.pdf}
\centering
  \caption{CoLA Error}
   \label{app:cola_err}
\end{subfigure}
\caption{The empirical evidence of mismatched objectives between  a standard low-rank factorization and task performance.
}
\label{app:err_per}
\end{figure}

==> tabs_figs/app_fig2.tex <==
\begin{figure} [htbp]
  \begin{subfigure}[b]{.49\textwidth}
   \centering
   \includegraphics[width=\textwidth]{figures/app_cola_rank.pdf}
       \caption{COLA}
       \label{app:rank:cola}
       \end{subfigure}
\begin{subfigure}[b]{.49\textwidth}
\includegraphics[width=\textwidth]{figures/app_ner_rank.pdf}
\centering
  \caption{NER (CoNLL-2003)}
   \label{app:rank:ner}
\end{subfigure}
  \begin{subfigure}[b]{.49\textwidth}
   \centering
   \includegraphics[width=\textwidth]{figures/app_rte_rank.pdf}
       \caption{RTE}
       \label{app:rank:0.rte}
       \end{subfigure}
\begin{subfigure}[b]{.49\textwidth}
\includegraphics[width=\textwidth]{figures/app_stsb_rank.pdf}
\centering
  \caption{STS-B}
   \label{app:rank:stsb}
\end{subfigure}
\caption{FWSVD+finetune versus SVD++finetune by varying the ratio of reserved ranks. The model with a rank ratio 1.0 indicates the full-rank reconstruction with the same accuracy as the original model.
}
\label{app:rank}
\end{figure}

==> tabs_figs/exp_temp_results.tex <==
albert-base-v1

cola_svd
group,1,2,3,4,5,6,7,8,9,10
eval_matthews_correlation, -0.0249, 0.0089, 0.1854, 0.1763, 0.2351, 0.3378, 0.4207, 0.3605, 0.4082, 0.1579
cola_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_matthews_correlation, 0.0111, 0.0029, 0.1338, 0.2737, 0.3551, 0.3917, 0.3969, 0.4148, 0.4174, 0.4594
mrpc_svd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.0, 0.0 0.0, 0.8183, 0.8253, 0.825, 0.8652, 0.8792, 0.8731 0.8731, 0.8908, 0.8298
mrpc_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.0, 0.3493, 0.6261, 0.8428, 0.8636, 0.8864, 0.8808, 0.8744, 0.8761, 0.8901
stsb_svd
group,1,2,3,4,5,6,7,8,9,10
eval_pearson, -0.0253, 0.3197, 0.7782, 0.7869, 0.8176, 0.8634, 0.8734, 0.8838, 0.873, 0.8256
stsb_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_pearson, -0.0582, 0.5067, 0.7536, 0.821, 0.8472, 0.8702, 0.8838, 0.8756, 0.8825, 0.887
sst2_svd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.5745, 0.7282, 0.797, 0.8257, 0.8257, 0.8693, 0.8578, 0.8681, 0.875, 0.8475
sst2_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.5172, 0.6101, 0.7672, 0.8349, 0.8716, 0.8658, 0.8727, 0.8704, 0.8853, 0.8853
mnli_svd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.3182 0.3182, 0.3525 0.3495, 0.6447 0.6544, 0.6337 0.6664, 0.7067 0.7037, 0.773 0.7714, 0.784 0.7797, 0.8053 0.8035, 0.7996 0.8048, 0.667 0.6706
mnli_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.3182 0.3186, 0.3853 0.3908, 0.6145 0.6238, 0.7268 0.7308, 0.7799 0.775, 0.7989 0.7947, 0.7977 0.7986, 0.8092 0.8031, 0.8137 0.8102, 0.8155 0.8182
qnli_svd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.4941 0.4941, 0.5596 0.5596, 0.777, 0.8159, 0.7964, 0.8664, 0.8794, 0.877, 0.8898, 0.6511
qnli_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.4946, 0.5111, 0.7505, 0.8082, 0.8656, 0.877, 0.886, 0.89, 0.8973, 0.8927
qqp_svd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.0089, 0.0205, 0.7356, 0.6393, 0.713, 0.8319, 0.8459, 0.8541, 0.8528, 0.8071
qqp_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.2791, 0.0079, 0.5898, 0.759, 0.8225, 0.84, 0.8514, 0.8541, 0.8555, 0.8571
ner_svd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.0409, 0.5101, 0.6409, 0.7213, 0.7845, 0.8629, 0.8846, 0.8863, 0.8926, 0.8456
ner_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.0103, 0.1428, 0.603, 0.761, 0.8561, 0.8748, 0.889, 0.907, 0.908, 0.9133


bert-base-uncased
cola_svd
group,1,2,3,4,5,6,7,8,9,10
eval_matthews_correlation, 0.0, 0.2359, 0.4248, 0.5222, 0.5731, 0.5788, 0.5591, 0.5523, 0.5859, 0.4092
cola_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_matthews_correlation, 0.0, 0.2016, 0.4666, 0.4724, 0.5702, 0.5725, 0.5751, 0.5472, 0.5551, 0.5778
mrpc_svd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.0, 0.0, 0.5735, 0.8699, 0.8589, 0.8907, 0.8758, 0.877, 0.8785, 0.6728
mrpc_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.0071, 0.0071, 0.8406, 0.859, 0.871, 0.8793, 0.8808, 0.8736, 0.8769, 0.8768
stsb_svd
group,1,2,3,4,5,6,7,8,9,10
eval_pearson, -0.0982, 0.5908, 0.8444, 0.8733, 0.878, 0.8856, 0.8833, 0.883, 0.884, 0.8278
stsb_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_pearson, 0.0282, 0.6052, 0.8598, 0.8756, 0.8797, 0.8841, 0.885, 0.8864, 0.885, 0.8854
sst2_svd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.4908, 0.8372, 0.8945, 0.9255, 0.9186, 0.9243, 0.9266, 0.9278, 0.93, 0.9209
sst2_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.5241, 0.8475, 0.9174, 0.9197, 0.9186, 0.9278, 0.922, 0.9266, 0.9289, 0.93
mnli_svd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.3512 0.3505, 0.4179 0.404, 0.7227 0.7098, 0.789 0.7787, 0.8284 0.8269, 0.8398 0.8387, 0.8407 0.8444, 0.8442 0.8442, 0.8451 0.8467, 0.8196 0.8245
mnli_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.3416 0.3356, 0.3895 0.3802, 0.7346 0.728, 0.8084 0.8034, 0.8422 0.8359, 0.8423 0.8422, 0.8397 0.8472, 0.8426 0.8467, 0.8458 0.8467, 0.8456 0.8472
qnli_svd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.4941, 0.5362, 0.7251, 0.8292, 0.8684, 0.8845, 0.9006, 0.9085, 0.9118, 0.8448
qnli_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_accuracy, 0.4946, 0.5288, 0.7465, 0.8332, 0.8788, 0.9006, 0.9114, 0.909, 0.912, 0.9103
qqp_svd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.1443, 0.6782, 0.7971, 0.8371, 0.8593, 0.8676, 0.8697, 0.8718, 0.8747, 0.8683
qqp_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.41, 0.6769, 0.8037, 0.8538, 0.8636, 0.8706, 0.8736, 0.8724, 0.8744, 0.8762
ner_svd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.026, 0.6366, 0.8859, 0.9156, 0.9201, 0.9282, 0.9353, 0.9361, 0.9389, 0.9231
ner_wsvd
group,1,2,3,4,5,6,7,8,9,10
eval_f1, 0.0183, 0.692, 0.8925, 0.9175, 0.9305, 0.9321, 0.9355, 0.9377, 0.9358, 0.9391

========
albert-base-v1
stsb_svd
RANK,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1
eval_pearson, -0.0189, -0.0351, 0.0258, -0.0067, -0.0727, 0.427, 0.6936, 0.7488, 0.8256, 0.8905
stsb_wsvd
RANK,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1
eval_pearson, -0.0608, 0.0674, 0.2469, 0.4581, 0.7452, 0.7929, 0.8332, 0.8728, 0.887, 0.8905

albert-large-v1
stsb_svd
RANK,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1
eval_pearson, 0.1142, 0.0704, 0.0594, -0.0717, -0.1334, -0.1244, -0.0602, -0.0667, 0.0482, 0.9013
stsb_wsvd
RANK,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1
eval_pearson, -0.0478, 0.0015, 0.0678, 0.15, 0.8042, 0.8433, 0.8727, 0.8861, 0.8897, 0.9013



========
NeMo
(dev other WER)	rank ratio	0.1	0.2	0.3	0.4	0.5	0.6	0.7	0.8	0.9	1
Conformer-CTC Large	#param	 36,511,361.00 	 50,611,841.00 	 64,712,321.00 	 78,812,801.00 	 93,189,761.00 	 107,290,241.00 	 121,390,721.00 	 135,491,201.00 	 149,591,681.00 	 163,968,641.00 
	SVD	1.00	1.00	0.99	0.78	0.35	0.18	0.10	0.08	0.06	0.05
	FWSVD	1.00	0.98	0.82	0.52	0.23	0.11	0.08	0.06	0.06	0.05
Conformer-CTC Medium	#param	 9,222,017.00 	 12,816,257.00 	 16,272,257.00 	 19,866,497.00 	 23,460,737.00 	 26,916,737.00 	 30,510,977.00 	 33,966,977.00 	 37,561,217.00 	 41,155,457.00 
	SVD	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	0.91	0.07
	FWSVD	1.00	1.00	1.00	0.96	0.73	0.38	0.17	0.10	0.08	0.07
	SVD ft 50e lr=0.01						0.12				
	FWSVD ft 50e lr=0.01						0.11				
Conformer-CTC Small	#param	 4,023,665.00 	 5,544,305.00 	 6,980,465.00 	 8,501,105.00 	 10,021,745.00 	 11,457,905.00 	 12,978,545.00 	 14,414,705.00 	 15,935,345.00 	 17,455,985.00 
	SVD	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	0.89	0.09
	FWSVD	1.00	1.00	1.00	0.99	0.92	0.67	0.32	0.16	0.11	0.09

==> tabs_figs/fig1_backup.tex <==
\begin{figure} %[htbp]
  \begin{subfigure}[b]{.49\textwidth}
   \centering
   \includegraphics[width=\textwidth]{figures/exp_fig1_COLA.pdf}
       \caption{COLA}
       \label{fig:rank:cola}
       \end{subfigure}
\begin{subfigure}[b]{.49\textwidth}
\includegraphics[width=\textwidth]{figures/exp_fig1_NER.pdf}
\centering
  \caption{NER (CoNLL-2003)}
   \label{fig:rank:ner}
\end{subfigure}
  \begin{subfigure}[b]{.49\textwidth}
   \centering
   \includegraphics[width=\textwidth]{figures/exp_fig1_RTE.pdf}
       \caption{RTE}
       \label{fig:rank:0.rte}
       \end{subfigure}
\begin{subfigure}[b]{.49\textwidth}
\includegraphics[width=\textwidth]{figures/exp_fig1_STSB.pdf}
\centering
  \caption{STS-B}
   \label{fig:rank:stsb}
\end{subfigure}
\caption{FWSVD versus SVD by varying the ratio of reserved ranks. The model with a rank ratio 1.0 indicates the full-rank reconstruction with the same accuracy as the original model (\ie, the $L^t$ in Figure \ref{fig:scheme}). Note that all the models here do not have fine-tuning after factorization. 
See Figure \ref{app:rank} in Appendix for the comparison of SVD and FWSVD with fine-tuning.
}
\label{fig:rank}
\end{figure}

==> tabs_figs/tab1_backup.tex <==

\begin{table}%[!tbp]
\centering
\caption{Results of CoNLL and GLUE benchmark. Note the AVG (average of GLUE tasks) excludes CoNLL.}
\label{tab:GLUE}
\renewcommand\tabcolsep{2.0pt}
\resizebox{1\textwidth}{!}{
\begin{tabular}
%{p{2.3cm}|c|p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}|p{0.7cm}}
{l|l|c|c|cccccccc|c}
\toprule
&Model& \#Param &  CoNLL &  CoLA &  MNLI &  MRPC &  QNLI &  QQP &  RTE &  SST-2 &  STS-B &  AVG \\ \midrule
Original&BERT$_{base}$ & 109.5M & 94.1 & 56.2 & 84.7 & 87.4 & 91.3 & 87.8 & 67.9 & 93.0 & 88.5 & 82.1 \\ \midrule
\multirow{ 2}{*}{Path-1}&DistilBERT & 67.0M & 93.2 & 49.8 & 82.2 & 88.7 & 89.3 & 86.7 & 58.5 & 90.4 & 86.1 & 79.0 \\
&MiniLMv2 & 67.0M & 92.2 & 43.3 & 84.0 & 89.1 & 90.6 & 86.7 & 67.5 & 91.4 & 88.1 & 80.1 \\ \midrule
\multirow{ 5}{*}{Path-2}&BERT-PKD & 67.0M & $-$ & 45.5 & 81.3 & 85.7 & 88.4 & 88.4 & 66.5 & 91.3 & 86.2 & 79.2 \\ 
&BERT+SVD & 66.5M & 12.0 & 2.7 & 35.6 & 61.4 & 37.2 & 60.0 & 52.4 & 76.7 & 26.8 & 44.1 \\
&\multicolumn{1}{r|}{+fine-tuning} 
& 66.5M & 92.4 & 40.5 & 82.8 & 84.1 & 89.6 & 87.3 & 61.0 & 91.0 & 85.7 & 77.7 \\
&BERT+FWSVD & 66.5M & 49.6 & 13.5 & 52.8 & 81.2 & 52.2 & 65.7 & 53.1 & 82.1 & 68.6 & 58.6 \\
&\multicolumn{1}{r|}{+fine-tuning} & 66.5M & 93.2 & 49.4 & 83.0 & 88.0 & 89.5 & 87.6 & 62.8 & 91.2 & 87.0 & 79.8 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tabs_figs/tab3.tex <==
\begin{table}
\centering
\caption{Average absolute reconstruction error of Group-9 and Group-10 in Figure \ref{fig:remove_group}.}
\begin{tabular}{l|cc|cc}
\toprule
{Average absolute }& \multicolumn{2}{c|}{Group-9} & \multicolumn{2}{c}{Group-10} \\ \cline{2-5}
 reconstruction error & SVD & WSVD & SVD & WSVD \\ \midrule
Whole matrix $\bar W$ & 1.34E-05 & 1.59E-05 & 7.77E-06 & 9.55E-06 \\
Top fisher columns $\bar W_f$ & 1.54E-05 & 4.75E-07 & 1.41E-05 & 2.19E-07 \\
\bottomrule
\end{tabular}
\end{table}
